Partitioned Sampling of Public Opinions Based on Their Social Dynamics

Public opinion polling is usually done by random sampling from the entire population, treating individual opinions as independent. In the real world, individuals' opinions are often correlated, e.g., among friends in a social network. In this paper, we explore the idea of partitioned sampling, which partitions individuals with high opinion similarities into groups and then samples every group separately to obtain an accurate estimate of the population opinion. We rigorously formulate the above idea as an optimization problem. We then show that the simple partitions which contain only one sample in each group are always better, and reduce finding the optimal simple partition to a well-studied Min-r-Partition problem. We adapt an approximation algorithm and a heuristic algorithm to solve the optimization problem. Moreover, to obtain opinion similarity efficiently, we adapt a well-known opinion evolution model to characterize social interactions, and provide an exact computation of opinion similarities based on the model. We use both synthetic and real-world datasets to demonstrate that the partitioned sampling method results in significant improvement in sampling quality and it is robust when some opinion similarities are inaccurate or even missing.

==> content/experiment.tex <==
\section{Experimental Evaluation}\label{section: experimental evaluation} 

In this section, we compare the sampling quality of
    partitioned sampling using greedy partitioning (\textsf{Greedy}) 
    and partitioned sampling using SDP partitioning\footnote{We use CVX package \cite{cvx,gb08} to solve the SDP programming.} (\textsf{SDP}) against 
	naive sampling (\textsf{Naive}) based on the \model{} model, using both synthetic and real-world datasets.
We describe major parameter settings for the experiments below, while leave the complete settings in
	the supplemental material due to the space constraint.

%We defer a full discussion of the implementation details to the appendix.
    
%To be specific, 
%we first describe the generation of our synthetic graphs, and show the comparison of various sampling methods and how graph structure and inward tendency affect the performance of the sampling methods in Section \ref{section:synthetic}.
%We then move on to the real-world dataset in Section \ref{section:realdata} to show
%	a method of learning the distribution of inward probabilities from online social networks,
%	and the performance of partitioned sampling on the real-world graph based on the learned
%	inward probabilities.

In our experiment, when the parameters of \model{} model are set, the simulation is done by (a) calculating the pairwise opinion similarities by Theorem \ref{theorem: similarity}, (b) running the partitioning algorithms to obtain the partition candidate, and (c) computing the expected variance $\E_M[\Var_S(\hat f)]$ by 
	Theorem~\ref{theorem:objective function}.
%In both synthetic and real-world datasets, we set $\mu^{(0)}$ to $0.5$.
%Notice that the value of $\mu^{(0)}$ has no effect on the results (Theorem \ref{theorem: similarity}).

%\subsection{Synthetic Dataset}\label{section:synthetic}

\begin{figure}[t] 
    \centering
    \def \mag {0.224}
    \subfigure[Synthetic graph ($100$ nodes)] {      
        \includegraphics[width=\mag\textwidth]{node100.eps}  \label{fig:small}
    }
    \subfigure[Synthetic graph ($\num{10000}$ nodes)] { \label{fig:cluster}     
        \includegraphics[width=\mag\textwidth]{cluster.eps} 
    }
    \subfigure[Synthetic graph ($\num{10000}$ nodes)] { \label{fig:inward}     
        \includegraphics[width=\mag\textwidth]{inward.eps}  
    }
    \subfigure[Inward probability distribution] { \label{fig:p distribution}     
        \includegraphics[width=\mag\textwidth]{p_distribution.eps}  
    }
    \subfigure[Weibo graph with $\lambda_i=1$] { \label{fig:lambda=1}     
        \includegraphics[width=\mag\textwidth]{nonpoisson.eps} 
    }
    \subfigure[Weibo graph with $\lambda_i$ set to the number of $v_i$'s tweets in a year] { \label{fig:poisson}     
        \includegraphics[width=\mag\textwidth]{poisson.eps}
    }
    
\end{figure} 

\textbf{Synthetic Dataset.} We use the planted partition model \cite{HiddenPartition} to generate undirected graphs, which aims at resembling the community structure in real-world social networks. 
Given $n$ vertices and $k$ latent disjoint groups,
    every edge $(v_i,v_j)$ is generated with a high probability $p_H$ if $v_i$ and $v_j$ are in the same latent 
    group, otherwise with a low probability $p_L$.


We generate two different sizes of synthetic graphs.
The small one includes $100$ nodes and $20$ latent groups,
and $p_H$, $p_L$ and $\lambda_i$ are set to $0.9$, $0.01$ and $1$, respectively.
The inward probability of each node is randomly chosen from $[0,0.01]$.
Fig \subref{fig:small} shows that,
	when the sample size $r$ is small, the performance of \textsf{SDP} and \textsf{Greedy} are similar to each other and both better than \textsf{Naive}.
When the sample size $r$ increases,
\textsf{Greedy} becomes much better than \textsf{Naive}, and \textsf{SDP} starts getting worse.
For the large synthetic graph with $10$k nodes and $500$ latent groups, 
    \textsf{SDP} is no longer feasible, thus we compare the
    improvement of \textsf{Greedy} against \textsf{Naive}.
In Fig \subref{fig:cluster},
    we range $p_H/p_L$
    and find that larger $p_H/p_L$ (more apparent clustering) indicates the better performance of our partitioned sampling.
When $p_H/p_L$ increases from $10^3$ to $10^5$, the improvement of expected sample variance increases rapidly.
When $p_H/p_L>10^5$, 
the improvement becomes saturated.
This is because the number of edges which cross different latent groups are so few that it decreases rather slowly and the graph structure is almost unchanged when $p_H/p_L$ increases further.
In Fig \subref{fig:inward},
we set all nodes' inward probabilities to be equal and vary them from $0.02$ to $0.8$.
The figure shows that the lower inward probability leads to the better performance of our partitioned sampling.
When the inward probability gets small, the improvement of expected sample variance increases rapidly.
This is because a lower inward probability means people interacting more with their friends
	and thus their opinions are correlated more significantly.
According to the above experiments, we conclude that
the larger $p_H/p_L$
and the lower inward probability 
make people's opinions more clustered and more correlated inside the clusters, and our partitioned
	sampling method works better for these cases.


\textbf{Real-World Dataset.}
We use the micro-blog data from \url{weibo.com} \cite{weibodata},
which contains $\num{100102}$ users and $\num{30518600}$ tweets within a one-year timeline from 1/1/2013 to 1/1/2014.
We treat the user following relationship between two users as a directed edge (with weight $1$).

We first learn the distribution of user's inward probabilities from the data.
We extract a series of users' opinions on $12$ specific topics (e.g., Microsoft, iPhone, etc.) by applying a keyword classifier and a sentiment analyzer \cite{sentiment} to the tweets.
We also collect their relationships and form a subgraph for each topic.
Then we use VIO model to fit the data by solving a minimization problem w.r.t. inward probabilities using gradient descent.
Fig \subref{fig:p distribution} shows the distribution of inward probabilities for 
	three of the topics, namely Spring Festival Gala ($68$ users), Microsoft ($66$ users) and iPhone ($59$ users), and the results for
	other topics are similar.
%The distributions among different topics are quite similar:
From these distributions, we observe that
(a) over $45\%$ inward probabilities locate in $[0, 0.2]$; 
(b) the probability that $p_i$ locates in $[0.8, 1]$ is the second highest;
(c) others almost uniformly locate in $[0.2, 0.8]$.
This indicates that in the real world, most people tend to adopt others' opinions,
which matches the intuition that people are often affected by others.
We manually look up those users who locate in $[0.8, 1]$, 
and find that most of them are media accounts and verified users.
This matches our intuition that those users always take effort to spread their 
	own opinions on the web but rarely adopt other people's opinions,
	hence they should have large inward probabilities.

Now we simulate our sampling methods on the Weibo graph.
We first remove the users who do not follow anyone iteratively,
    and get the graph including $\num{40787}$ nodes and $\num{165956}$ directed edges.
We generate each user's inward probability following the distribution we learned.
We use two different settings for opinion updating rates:
one is to set $\lambda_i=1$ for all $i\in[n]$;
the other is to set $\lambda_i$ to the number of $v_i$'s tweets in a year.
The improvement of \textsf{Greedy} against \textsf{Naive}
with two different updating rate settings are similar as shown in Fig \subref{fig:lambda=1} and \subref{fig:poisson}.
In particular, if we fix $\E_M[\Var_S(\hat f)]$ to be $\num{3.86e-5}$, \textsf{Greedy} needs $4794$ samples while \textsf{Naive} needs $8000$ samples (saving $40.1\%$) in Fig~\subref{fig:lambda=1},
and \textsf{Greedy} needs $4885$ samples while \textsf{Naive} needs $8000$ samples (saving $38.9\%$) in Fig~\subref{fig:poisson}.
This indicates that partitioned sampling greatly improves the sampling quality,
    and the sample size saving is more apparent when
    the expected sample variance gets smaller (i.e., the requirement of sampling quality is higher).
Moreover, in order to test the performance of partitioned sampling with missing and inaccurate opinion similarities,
    we artificially remove all the opinion similarity information between disconnected nodes (set as 0.5), and 
    perturb each rest similarity $\sigma_{ij}$ with a random noise
    in the range of $\pm (0.1+30\% \cdot \sigma_{ij}) $.
%     $\pm 0.1$ plus relative noise $\pm 30\%$.
Fig \subref{fig:lambda=1} and \subref{fig:poisson} show that \textsf{Greedy} using the above perturbed similarities (denoted as \textsf{Greedy\_P}) is very close to \textsf{Greedy}, and still has a 
	significant improvement against naive sampling.

In conclusion, the experimental results demonstrate the excellent performance of our partitioned sampling 
	method both on synthetic and real-world datasets, even when the opinion similarities are missing or inaccurate.
%The figures also indicate that our partitioned sampling method is consistently better than naive sampling method regardless of the updating rate settings.

%In conclusion, the results are consistent with the results from synthetic graphs in demonstrating the better
%performance of partitioned sampling method.

%\wei{I did not see the graph size, like the number of nodes and the number of edges, after the cleanup if any.}


==> content/introduction.tex <==
\section{Introduction}

Public opinion is essential nowadays for governments, organizations and companies to make decisions on their policies, strategies, products, etc.
%Public opinion polling is a main tool for governments, organizations and companies to gather public sentiments on the policies, strategies, products, etc., which play important role in decision making.
The most common way to collect public opinions is polling, typically
	done by randomly sampling a large number of individuals from the entire population and then interviewing them by telephone.
This naive method is unbiased, but conducting interviews is very costly.
%Opinion poll needs to be accurate and unbiased, and thus it is usually done by randomly sampling a large enough number of individuals from the entire population, but this is a costly effort.
On the other hand, in recent years, more and more online social media data are available and have been used to predict public opinions on certain issues.
Such predictions cost less human effort, but they are usually biased
	and may lead to incorrect decisions.
Thus keeping the estimation unbiased while saving the cost becomes an important task to pursue.
%Therefore, saving the cost on unbiased sampling while keeping the same sampling quality is an important task to pursue.

In this paper, we utilize individuals' social interactions (potentially learned from social media data) to improve the unbiased sampling method.
Our motivation is from the fact that people's opinions are often correlated, especially among friends in the social network, due to their social interactions in terms of the homophily and influence effects \cite{Homophily,Duncan,Kleinberg}.
These correlations are partially known in the big data era.
For example, many online social media and social networking sites provide publicly available social interaction data and user's sentiment data, and companies also have large amounts of data about their customer's preference and their social interaction. 
Our idea is to partition individuals into different groups by utilizing these prior knowledge,
	 such that people within a group are likely to hold the same opinions.
We can then sample very few people in each group and aggregate the sampling results together to achieve an accurate estimation.
We call this {\em partitioned sampling} method.

We formulate the above idea as an optimization problem.
In particular, we first 
	characterize individuals' opinions as random variables. %, which are often
	%correlated due to their social interactions.
We then specify our objective as minimizing
	the expected sample variance of the estimate, and
	define the statistical measure of pairwise {\em opinion similarity} as the input.
Our analysis later shows that this input is enough to fully determine the solution
	of the optimization problem, named the
	{\em Optimal Partitioned Sampling (OPS)} problem (Section \ref{section: formulating the problem}).

We solve the OPS problem in two steps (Section \ref{section: solving the OPS problem}).
First, we show that 
    the best partition is always a {\em simple partition}, 
    meaning that each group contains only one sample.
Second, we use people's opinion similarities to construct a weighted graph and 
    reduce the OPS problem to the Min-$r$-Partition problem.
    %a graph partitioning problem, which is a special case of the well-studied Min-$r$-Partition problem.
We adapt a semi-definite programming algorithm and a heuristic algorithm %for the dual problem of Min-$r$-Partition 
	to solve our optimization problem.
%We adopt a semi-definite programming algorithm for the dual problem of Min-$r$-Partition to solve the OPS problem, and further propose an efficient greedy partitioning algorithm to work on larger graphs.
We further show that partitioned sampling using any balanced simple partition where group sizes are the same
	always out-performs naive sampling method, and thus balanced simple partition is always safe to use even if we only have
	partial or inaccurate opinion similarity information.

%\wei{talk about balanced partition always better than naive sampling, may also refer to Facebook and polling applications}

Next we adapt existing opinion evolution models and propose the Voter model with Innate Opinions (VIO) based
	on social network interactions (Section \ref{section: opinion evolution model and opinion similarity}).
%To efficiently compute pairwise opinion similarities,
%	we adapt existing opinion evolution models and propose the Voter model with Innate Opinions (VIO).
We provide an exact computation of opinion similarities in the steady state of
	the model, which is novel in the study of such models.



Finally, we conduct experiments on both synthetic and real-world datasets
to demonstrate the effectiveness and robustness of our partitioned sampling method
(Section \ref{section: experimental evaluation}).

In summary, our contributions include: 
(a) proposing the partitioned sampling method to
improve sampling quality based on opinion similarities
and formulating it as an optimization problem, 
(b) precisely connecting the OPS problem to
the Min-$r$-Partition problem and providing efficient algorithms 
for the OPS problem,
and 
(c) adapting an opinion evolution model and providing
an exact computation of opinion similarities based on the model.

Due to space constraint, we put the mathematical proofs and technical details into the supplemental material.

\textbf{Related Work.}
There are a number of sampling methods in the literature.
The most related method is stratified sampling
 \cite{bethel1986optimum,bethel1989sample,chromy1987design,cochran2007sampling,kozak2007modern,keskinturk2007genetic,ballin2013joint}.
The entire population is first stratified into homogeneous atomic strata based on individuals' profiles (e.g., age, gender, etc.),
	and then they may be combined to a final stratification and 
	subsample size in each stratum is allocated to minimize sample variance.
Conceptually, our partitioned sampling method is similar to stratified sampling, but there are some important differences.
First, stratified sampling partitions individuals based on their profiles, which may not imply opinion similarity, while we partition individuals
	directly based on opinion similarity, and thus our method is more accurate and flexible.
Second, the technical treatments are different. Stratified sampling treats individual opinions as fixed and unknown, 
	and requires the (estimated) mean and standard deviation of opinions in each stratum to bootstrap the
	stratified sampling, while we treat individual opinions as random variables, and use pairwise opinion 
	similarities for partitioned sampling.
	

%The entire population is first stratified into several homogeneous atomic strata by some attributes (e.g., age, gender, nationality, etc.),
%and they are combined to a final stratification according to the limited number of strata.
%Then subsample size in each stratum is allocated to minimize sample variance.
%Some work \citep{bethel1986optimum,bethel1989sample,chromy1987design} focus on optimizing the allocation while the stratification is given, and some \citep{ballin2013joint,kozak2007modern,keskinturk2007genetic} focus on simultaneously optimizing the stratification and allocation.
%In stratified sampling, individuals' opinions are regarded as fixed but unknown, 
%and the optimization task requires the standard derivation of each stratum known ahead, which is hard to obtain before sampling in practice.
%On the other hand, stratified sampling works effectively only under the circumstance that people with same attributes are likely to hold same opinions,
%which does not always stand in the real world.
%%For the stratifying, although the motivation is to make people within stratum be homogeneous, actually each atomic strata is generated by the attribution, which may lead to large standard deviation within stratum.
%%For the allocating, the optimization task requires the standard derivation of each stratum known ahead, which is hard to obtain before sampling in practice.
%By comparison, our partitioned sampling also optimizes the stratification and allocation jointly, 
%but does not need any information about the sampling at present.
%Instead, we only add an acceptable assumption that we have some prior stochastic knowledge about people's opinions.
%Moreover, we directly use opinion similarity to determine the stratification instead of stratifying by attributes.
%

Among studies on social interaction based sampling, \citet{SocialSampling} utilize social network connections to facilitate sampling.
However, their method is to ask the voter being sampled to return the estimate of her friends' opinions,
    %However, their method is to explicitly ask the voter being sampled to return additional information about their friends' opinions,
    which changes the polling practice. 
In contrast, we still follow the standard polling practice and only use implicit knowledge on opinion similarities to improve sampling quality.
%These two ideas are orthogonal and could be potentially combined together.
%\huang{del respondent-driven sampling}
%Another popular social-interaction based sampling method is respondent-driven sampling \citep{respondent1,respondent2},
%    which gets individuals to refer those they know.
%It is an adaptive sampling method and designed for estimating the proportion of those very small and hard-to-reach groups such as drug injectors, which are hard to deal with by normal sampling methods.
%Our partitioned sampling method is not limited by the size of the target population.
\citet{DebiasingSocial} consider the task of estimating 
	people's average innate opinion by removing their social interactions,
	which is opposite to our task --- we want to utilize opinion interactions for more efficient sampling of final expressed opinions which are counted in opinion polls.
%\citet{DebiasingSocial} study the task of removing the correlations among individual's opinions due to their social interactions to obtain the average {\em original innate opinion}. 
%Their task is to utilize the wisdom of the crowd for extracting the latent {\em independent} opinions of individuals.
%
Graph sampling methods \cite{gjoka2010walking,kurant2011walking} aim at achieving unbiased uniform sampling on
	large scale networks when the full network is not available, which is orthogonal to our partitioned sampling
	approach and could be potentially combined together. 

Various opinion evolution models have been proposed in the literature
\cite{DiscreteOpinion,DebiasingSocial,OpinionMaximization,Li0WZ15}.
Our \model{} model is adapted from the voter model \cite{VoterModel} and its extension with stubborn agents \cite{DiscreteOpinion}.
%But to the best of our knowledge, we are the first to develop the exact computation of opinion correlations and
%	similarities in such models.
%%The models in \citep{DebiasingSocial,OpinionMaximization} also distinguish between innate opinions and expressed opinions, 
%%however, their models are deterministic, and thus their analyses do not apply to our stochastic analysis on the similarities and correlations between final expressed opinions.
%We give an random-walk view of opinion evolution, and propose an exact and an efficient computations of opinion correlations and similarities.

Graph partitioning has been well studied, and numerous problem variants and algorithms exist.
In this paper, we reduce the OPS problem to the Min-$r$-Partition problem, 
which was first formulated by \citet{sahni1976p}.
%\citet{kann1997hardness} further show that it is NP-hard to approximate to within a factor of $|V|^{2-\epsilon}$ for $r>2$.
%\huang{quoted from their paper: For the Min k-Partition problem, we show that for $k > 2$ and for every $\epsilon > 0$, there exists
%    a constant $\alpha$ such that the problem cannot be approximated within $\alpha |V|^{2-\epsilon}$}
%which is the problem of partitioning the graph in to $r$ groups and minimizing the total weights of edges whose two ends are in the same group.
%Min-$r$-Partition is NP-hard to approximate to within any finite factor, 
To the best of our knowledge, there is no approximation or heuristic algorithms for Min-$r$-Partition.
Thus we adapt a state-of-art approximation algorithm for the dual problem (Max-$r$-Cut) to solve the OPS problem \cite{maxkcut}.
We also propose a greedy algorithm for large graphs, which takes the idea from a heuristic algorithm for Max-$r$-Cut \cite{zhu2013max}.
%the semi-definite programming algorithm for the dual problem of Min-$r$-Partition (i.e., Max-$r$-Cut), proposed by \citet{maxkcut} for solving our OPS problem.



==> content/model.tex <==
\section{Opinion Evolution Model}\label{section: opinion evolution model and opinion similarity}

We adapt the well-known {\em voter model} to describe social dynamics \cite{VoterModel,DiscreteOpinion}.
Consider a weighted directed social graph $G=(V, A)$ where $V=\{v_1, v_2, \dots, v_n\}$ is the vertex set and $A$ is the weighted adjacency matrix. 
%An edge $(v_i, v_j)$ represents the opinion influence relationship from $v_j$ to $v_i$.
Each node is associated with both an {\em innate opinion} and an {\em expressed opinion}. 
The innate opinion remains unchanged from external influences, while the expressed opinion could be shaped by the opinions of one's
neighbors, and is the one observed by sampling.
At initial time, 
each node $v_i$ generates its innate opinion $f^{(0)}(v_i) \in \{0,1\}$ from an i.i.d.\ Bernoulli distribution with expected value $\mu^{(0)}$.
The use of i.i.d.\ distribution for the innate opinion is due to the lack of prior knowledge on a brand-new 
topic, and is also adopted in other models \cite{SocialSampling}.
When $t>0$, each node $v_i$ updates its expressed opinion $f^{(t)}(v_i) \in \{0,1\}$ independently according to a Poisson process with updating rate $\lambda_i$: 
at its Poisson arrival time $t$, node $v_i$ sets $f^{(t)}(v_i)$ to its 
innate opinion with an {\em inward probability} $p_i>0$, or with probability $(1-p_i)A_{ij}/\sum_{k=1}^{n} A_{ik}$, adopts its out-neighbor $v_j$'s expressed opinion
$f^{(t)}(v_j)$.
We call the model  {\em Voter model with Innate Opinions (\model{})}.

%We adapt the well-known {\em voter model} to describe social dynamics \cite{VoterModel,DiscreteOpinion}.
%Consider a weighted directed social graph $G=(V, A)$ where $V=\{v_1, v_2, \dots, v_n\}$ is the vertex set and $A$ is the weighted adjacency matrix.
%Each node $v_i$ possesses an {\em innate opinion} $f^{(0)}(v_i) \in \{0,1\}$, which remains unchanged from external influences, and
%	is generated from an i.i.d.\ Bernoulli distribution with expected value $\mu^{(0)}$.
%The use of i.i.d.\ distribution for the innate opinion is due to the lack of prior knowledge on a brand-new 
%	topic, and is also adopted in other models \cite{SocialSampling}.
%Each node $v_i$ also has an {\em expressed opinion} $f^{(t)}(v_i)\in\{0,1\}$ at time $t$, which could be shaped by
%	other nodes' expressed opinions and $v_i$'s innate opinion. % and change over time.
%Each node $v_i$ updates its expressed opinion independently according to a Poisson process with updating rate $\lambda_i$. At its Poisson arrival time, node $v_i$ either sticks to its 
%innate opinion with an {\em inward probability} $p_i>0$, or with probability $(1-p_i)A_{ij}/\sum_{k=1}^{n} A_{ik}$, adopts the expressed opinion
%    of its out-neighbor $v_j$.
%We call the model  {\em Voter model with Innate Opinions (\model{})}.


    
    
The \model{} model reaches a steady state if the joint distribution 
of all node's expressed opinions no longer changes over time.\footnote{The \model{} model has a unique joint
	distribution for the final expressed opinions. See supplemental material for the proof.} 
We use notation $f^{(\infty)}(v_i)$ to represent the steady-state expressed opinion of node $v_i$, which is a random variable.
We assume that opinion sampling is done in the steady state, which means that people have sufficiently communicated within the social network.

To facilitate analysis of the VIO model, %\footnote{We provide a full analysis of the VIO model in the supplemental material.}, 
    we take an equivalent view of the \model{} model as {\em coalescing random walks} on an augmented graph $\overline G = (V\cup V', 
E\cup \{e_1^\prime, e_2^\prime, \dots, e_n^\prime\})$, where $V^\prime=\{v_1', v_2', \dots, v_n'\}$ is a copy of $V$, $E$ is the edge set of $G$ and $e_i'=(v_i, v_i')$ for all $i$. In this viewpoint, we have $n$ walkers randomly wandering on $\overline G$ ``back in time'' as follows. At time $t$, all walkers are separately located at $v_1, v_2, \cdots, v_n$.
Suppose before time $t$, $v_i$ is the last node who updated its expressed opinion at time $\tau<t$,
then the $n$ walkers stay stationary on their nodes from time $t$ until time $\tau$ ``back in time''. At time $\tau$, the walker at node $v_i$ takes a walk step:
she either walks to $v_i$'s out-neighbor $v_j\in V$ with probability $(1-p_i)A_{ij}/\sum_{k=1}^{n} A_{ik}$, 
    or walks to $v_i' \in V'$ with probability $p_i$.
If any walker (e.g., the walker starting from node $v_i$) walks to a node (e.g., $v_k'$) in $V'$, 
    then she stops her walk.  In the \model{} model language, this is equivalent to saying that $v_i$'s opinion at time $t$ is determined
    by $v_k$'s innate opinion, namely $f^{(t)}(v_i)=f^{(0)}(v_k)$.
If two random walkers meet at the same node in $V$ at any time, they 
walk together from now on following the above rules (hence the name {\em coalescing}).
Finally, at time $t=0$, if the walker is still at some node $v_i\in V$, she always walks to
$v_i' \in V'$.

We now define some key parameters based on the coalescing random walk model, which will be directly used for computing the opinion similarity later. 

\begin{restatable}{definition}{walkparamdef}\label{def:walkparam}
%\begin{definition} 
    Let ${\cal I}_{ij}^\ell$ denote the event that two random walkers starting from $v_i$ and $v_j$ at time $t=\infty$ eventually meet and the first node they meet at is $v_\ell\in V$.
    Let $Q$ be the $n\times n$ matrix where $Q_{ij}$ denotes the probability
    that a random walker starting from $v_i$ at time $t=\infty$
    ends at $v_j^\prime \in V'$.
%\end{definition}
\end{restatable}	

\begin{restatable}{lemma}{walkparam}\label{lemma:walkparam}
    For $i,j,\ell\in [n]$, $\Pr\left[{\cal I}_{ij}^\ell\right]$ is the unique solution of the following
    linear equation system:
    \begin{equation*}
        \Pr\left[{\cal I}_{ij}^\ell\right]=
        \begin{cases}
            0, & i=j\neq \ell, \\
            1, & i=j=\ell,\\
            \sum_{a=1}^n \frac{\lambda_i (1-p_i) A_{ia} } {(\lambda_i+\lambda_j)d_i} \Pr[{\cal I}_{a j}^\ell] \\\quad
            +\sum_{b=1}^n \frac{\lambda_j (1-p_j) A_{jb} } {(\lambda_i+\lambda_j)d_j} \Pr[{\cal I}_{i b}^\ell]
            , & i\neq j,
        \end{cases}
    \end{equation*}
    where $d_i=\sum_{j=1}^n A_{ij}$ is $v_i$'s weighted out-degree.
    In addition, matrix $Q$ is computed by
    \begin{equation*}
        Q=\left(I-\left(I-P\right)D^{-1}A\right)^{-1}P,
    \end{equation*}
    where  $P=\diag(p_1, \dots, p_n)$ and $D = \diag(d_1, \dots, d_n)$
    are two diagonal matrices, and matrix $I-\left(I-P\right)D^{-1}A$ is invertible
    when $p_i>0$ for all $i\in [n]$.
\end{restatable}

Our main analytical result concerning the \model{} model is the following exact computation of pairwise opinion correlation, which directly leads to opinion similarity:

\begin{restatable}{lemma}{correlation}\label{lemma:correlation}
    For any $i,j\in [n]$, opinion correlation $\c_{ij}$ in the steady state is 
    equal to the probability that two coalescing random walks starting from $v_i$ and $v_j$ at time $t=\infty$ end at the same absorbing node in $V^\prime$.
    Moreover, opinion correlation $\c_{ij}$ can be computed by
    \begin{align*}
        \c_{ij}&=\Cor_M\left(f^{(\infty)}(v_i),f^{(\infty)}(v_j)\right) \\
        &= \sum_{k=1}^n Q_{ik}Q_{jk} + \sum_{\ell=1}^n\Pr\left[{\cal I}_{ij}^\ell\right]\left(1-\sum_{k=1}^n Q_{\ell k}^2\right)
    \end{align*}
    where ${\cal I}_{ij}^\ell$ and $Q$ are defined in Definition \ref{def:walkparam}, and
    $\Pr\left[{\cal I}_{ij}^\ell\right]$ and $Q$
    are computed by Lemma \ref{lemma:walkparam}.
\end{restatable}

\begin{restatable}{theorem}{similarity}\label{theorem: similarity}
	For any two nodes $v_i$ and $v_j$, their opinion similarity $\s_{ij}$ in the steady state of the \model{} model is equal to:
	$$\s_{ij}=1-2\mu^{(0)}(1-\mu^{(0)})(1-\c_{ij})$$
	where opinion correlation $\c_{ij}$ is computed by Lemma \ref{lemma:correlation}.
\end{restatable}

Notice that for partitioning algorithms, we only need $1-\s_{ij}$ as the edge weight and by the above theorem this weight value is proportional to $1 - \rho_{ij}$, which means the exact value of $\mu^{(0)}$ is irrelevant for partitioning algorithms.
In the supplemental material, we will provide an efficient computation of all pairwise opinion correlations 
	with running time $O(nm R)$ by
	a carefully designed iterative algorithm,
	where $m$ is the number of edges of $G$ which is commonly sparse, and $R$ is the number of iterations. 
We further remark that the correlations are calculated offline based on the existing network and historical data, 
	and thus the complexity compared to the sampling cost of telephone interview or network survey is relatively small. 
%Moreover, by Theorem \ref{thm:balancedpartition}, even if we save the offline computation cost by sacrificing the accuracy of correlations, we can still achieve better performance than naive sampling using balanced partitions.
	%\liang{which is better? previous expression for the last sentence:Moreover, according to Theorem \ref{thm:balancedpartition}, even if we cannot accurately estimate all correlations 
		%when the offline computation cost is high, we can still achieve better sampling performance using balanced partition.}

In the supplemental material, we further extend the VIO model to include (a) non-i.i.d. distributions of the innate opinions, and (b) negative edges as in
	the signed voter model \cite{Li0WZ15}.


==> content/package.tex <==
\usepackage{soul}
\usepackage[normalem]{ulem}
%\usepackage{hyperref}
\usepackage{url}
\usepackage{array}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thm-restate}
\usepackage{enumitem}
\usepackage{algorithm}
\usepackage{graphicx}
\usepackage[scriptsize,tight]{subfigure}
%\usepackage{caption}
%\usepackage{subfig}
\usepackage{algorithmicx,algpseudocode}
%\hypersetup{colorlinks=true, linkcolor=blue, citecolor=blue, anchorcolor=blue, urlcolor=black}  % link color
%\DeclareUrlCommand{\url}{\def\UrlFont{\color{black}\ttfamily}}  % url color
\usepackage{tikz}   % drawing package
\usetikzlibrary{calc}
\usepackage{epstopdf}   % Compile with pdflatex even if only .eps fig is given
%\usepackage[numbers,sort&compress]{natbib}
\usepackage{ifthen}
\usepackage{sistyle}
\SIthousandsep{,}
%\allowdisplaybreaks
\usepackage{float}
\graphicspath{{figure/}}

% personal definition
\DeclareMathOperator{\E}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}
\DeclareMathOperator{\Var}{\mathrm{Var}}
\DeclareMathOperator{\Cor}{\mathrm{Cor}}
\DeclareMathOperator{\Cov}{\mathrm{Cov}}
\DeclareMathOperator{\Cut}{\mathrm{Cut}}
\DeclareMathOperator{\OPT}{\mathrm{OPT}}
\DeclareMathOperator{\diag}{\mathrm{diag}}
\DeclareMathOperator{\Vol}{\mathrm{Vol}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
%\renewcommand\arraystretch{1.8}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% Debug 
\newcommand{\onlyarxiv}[1]{{\color{green!30!black}\uline{#1}}}
\newcommand{\onlypaper}[1]{{\color{blue!30!black}\uline{#1}}}
\newcommand{\wei}[1]{{\color{blue!50!black}  [\text{Wei:} #1]}}
\newcommand{\liang}[1]{{\color{brown!60!black} [\text{Liang:} #1]}}
\newcommand{\huang}[1]{{\color{magenta} [\text{Weiran:} #1]}}
\newcommand{\pending}[1]{{\color{magenta} [\text{Pending:} #1]}}
\newcommand{\npending}[1]{{\color{magenta} [\text{unPending:} #1]}}
\pagestyle{plain}
\pagenumbering{arabic}
\setstcolor{magenta}
\setul{}{2pt}

% Hide copyright info
\nocopyright

% micro for symbols
\newcommand{\e}{\mu}    % expected value
\renewcommand{\c}{\rho}         % correlation
\newcommand{\s}{\sigma}         % similarity
\newcommand{\model}{VIO}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


==> content/problem.tex <==
\section{Formulating the OPS Problem}\label{section: formulating the problem}

We consider a vertex set $V$ from a social network graph 
    containing $n$ vertices (or nodes) $v_1, v_2, \dots, v_n$.
Each vertex represents a person in the social network, 
    and has a binary opinion on some topic of interest. 
%We use $f_i\in\{0,1\}$ to denote $v_i$'s opinion.
%\st{, and then the average opinion can be formulated by $\bar f=\left. \sum_{i=1}^n f_i\middle/n\right.$.}
Our task is to estimate the average opinion of all individuals in the social network with sample size budget $r$. 
Let $f:V\rightarrow\{0, 1\}$ denote the opinion function, 
    i.e., we wish to estimate the fraction $\bar f = \frac{1}{n} \sum_{i=1}^n f(v_i)$.
The {\em naive sampling} method simply picks $r$ nodes uniformly at random with replacement 
	from $V$ to ask their opinions 
	and takes the average of sampled opinions as the estimate, as denoted below:
	$\hat f_{\it naive} (V,r) = \frac{1}{r} \sum_{i=1}^r f(x_i)$, where $x_i$ is the $i$-th sampled node.

%\newcounter{method}
%
%\begin{algorithm}[t]
%    \floatname{algorithm}{Method}
%    \caption{Naive Sampling}\refstepcounter{method}\label{al:naive}
%    \begin{algorithmic}[1]
%        \Require Vertex set $V$, sample size $r$.
%        \State Choose $r$ sample nodes $x_1$, $x_2$, \dots, $x_r$ from $V$ uniformly at random with replacement.
%        \State \textbf{Output:} $\hat f_{\it naive} (V,r) = \frac{1}{r} \sum_{i=1}^r f(x_i)$.
%    \end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}[t]
%    \floatname{algorithm}{Method}
%    \caption{Partitioned Sampling}\refstepcounter{method}\label{al:partitioned}
%    \begin{algorithmic}[1]
%        \Require Partition $\mathcal{P}=\{(V_1,r_1), (V_2,r_2), \dots, (V_K,r_K)\}$.
%        \For{$k\gets 1$ \textbf{to} $K$}
%        \State  Do naive sampling in $V_k$, \Return $\hat f_{\it naive} (V_k,r_k)$.
%        \EndFor
%        \State \textbf{Output:} $\hat f_{\it part}({\cal P}) =  \sum_{k=1}^K \frac{|V_k|}{|V|} \cdot \hat f_{\it naive} (V_k,r_k)$.
%    \end{algorithmic}
%\end{algorithm}

In this paper, we propose a general sampling framework called {\em partitioned sampling}.
%We then utilize the partial knowledge (i.e., people's opinion expectations and correlations) 
%(e.g., learned from historical voting data)
%to find the best partition for partitioned sampling.
Formally, we first partition the whole vertex set into several disjoint subsets (called {\em groups}), 
%    such that each vertex is included in one and only one of the groups, 
    and then allocate subsample size of each group.
We use $\mathcal{P}=\{(V_1,r_1),$ $(V_2,r_2), \dots, (V_K,r_K)\}$ to represent such a partition, 
    where $V_1$, $V_2$, \dots, $V_K$ are groups, 
    and $r_k$ is the subsample size of group $V_k$.
Next, we do naive sampling inside each group $V_k$ with its subsample size $r_k$.
Finally, we estimate the average opinion of the population
    by taking a weighted average of all subsampling results, 
    with weights proportional to group sizes:  
    $\hat f_{\it part}({\cal P}) =  \sum_{k=1}^K \frac{|V_k|}{|V|} \cdot \hat f_{\it naive} (V_k,r_k)$.
%We use $\hat f_{\it part}({\cal P})$ to denote the final estimate of partitioned sampling using partition $\cal P$.
Notice that naive sampling is a special case of partitioned sampling with $\mathcal{P}=\{(V,r)\}$.
%Before using partitioned sampling framework to design the efficient sampling method, we first show its unbiasedness in the following proposition.
One can easily verify that partitioned sampling is unbiased (see Supplemental Material).

%\begin{restatable}{proposition}{unbiased}
%    (Unbiasedness) Partitioned sampling is unbiased.
%    %Specifically, for any partition $\mathcal{P}$, $\E \left[\hat f_{\it part}(\mathcal{P})\right]=\bar f$.
%\end{restatable}
%\begin{proof}
%    For any partition $\mathcal{P}=\{(V_1, r_1),\ldots,(V_K,r_K)\}$,
%    according to the output formulation of Method \ref{al:partitioned},
%    \begin{align*}
%    &\E \left[\hat f_{\it part}(\mathcal{P})\right]
%    = \sum_{k=1}^K  \frac{|V_k|}{|V|} \E \left[\hat f_{\it naive}(V_k,r_k)\right]\\
%    &=\frac{1}{|V|} \sum_{k=1}^K  |V_k| \sum_{v_i\in V_k}\frac{f(v_i)}{|V_k|}
%    =\frac{\sum_{i=1}^n f(v_i)}{|V|}
%    =\bar f.
%    \end{align*}
%    Notice that naive sampling in any group $V_k$ is unbiased, thus $\E [\hat f_{\it naive}(V_k,r_k)]$ is equal to the average opinion of the people in $V_k$ (second equality above).
%    Therefore partitioned sampling is unbiased.
%\end{proof}

Intuitively, the advantage of using partitioned sampling is that, 
    if we partition individuals such that people likely holding the same opinions are partitioned into the same group, 
    then we can sample very few people in each group to get an accurate estimate of the average opinion of the group, 
    and aggregate them to get a good estimate of population mean.
To implement this idea, we assume that some prior knowledge about people's opinions and their
	similarities is available before sampling.
%Such prior knowledge %about people's opinions and their similarities 
%    can be derived from the past history of people's expressed opinions which organizations or online social networks have, 
%    or from their social interaction dynamics.
Based on these knowledge, our goal is to find the best partition for partitioned sampling which achieves the best sampling quality.

Our first research challenge is how to rigorously formulate the above intuition into an optimization problem.
To meet this challenge, we need to answer (a) which objective function is the appropriate one for the optimization problem, 
    and (b) which representation of the prior knowledge about people's opinions and their similarities 
    can be used as the input
    to the optimization problem.
%	what is the appropriate representation about people's knowledge and their similarities that can be used as the input
%	to the optimization problem to enable solving the problem.
	
We first address the objective function.
When all individuals' opinions $f(v_1), f(v_2), \dots, f(v_n)$ are fixed (but unknown), 
the effectiveness of an unbiased randomized sampling method is measured by the standard sample variance $\Var(\hat{f})$, 
where $\hat{f}$ is the estimate.
The smaller the sample variance, the better the sampling method.
When the prior statistical knowledge about people's opinions is available, effectively we treat
	opinions $f(v_1), f(v_2), \dots, f(v_n)$ as random variables, and the prior knowledge is
	some statistics related to the joint distribution of these random variables.
In this case, the best sampling method should minimize the {\em expected sample variance} $\E[\Var(\hat{f})]$, 
where the expectation is taken over the randomness from the joint distribution of people's opinions.
For clarity, we use $\E_M[\Var_S(\hat{f})]$ to represent $\E[\Var(\hat{f})]$, where
	subscript $M$ (standing for ``model'') represents the randomness from the
	joint distribution model of opinions, and subscript $S$ (standing for ``sampling'') represents sample randomness
	from the sampling method.
\footnote{One may propose to use the total variance $\Var_{M,S}(\hat f)$ as the objective function. %combining randomness from both the joint distribution and the sampling method. 
    In the supplemental material, we show that they are equivalent for the optimization task.}
%Therefore, our objective function is settled as minimizing the expected variance $\E_M[\Var_S(\hat{f})]$.

%We now answer the question of what kind of statistical knowledge about the joint distribution of people's opinions %$f(v_1), f(v_2), \dots, f(v_n)$
%	are needed as the inputs to enable the minimization of $\E_M[\Var_S(\hat{f})]$.
We now discuss the input to the optimization task. 
The full joint distribution of $f(v_1), f(v_2), \dots, f(v_n)$ requires
	an exponential number of parameters and is infeasible as the input.
%Naively, we could use the full joint distribution of $f(v_1)$, $f(v_2)$, \dots, $f(v_n)$ as the input, but
%	it requires an exponential number of parameters and is infeasible.
%
%First, note that these random variables are not mutually independent,
%since people's opinions are often correlated. %
%%, and partitioned sampling is based on the very fact about the existence of these correlations and would be useless if all people's opinions are independent.
%Thus, to fully characterize the joint distribution, we may need an exponential number of parameters, which is definitely infeasible in practice.
Then notice that the objective function only involves first two moments, which suggests us to use the expectations and pairwise correlations of people's opinions 
%(corresponding to the first two moments of the joint distribution)
	as the inputs.
Indeed we find that these knowledge is good enough to fully characterize the optimization problem. %we need to solve.
However, we further discover that a weaker and more direct type of statistics would be 
    enough to enable the %equivalent in terms of fully charactering the
	optimization problem, which we formally define as pairwise opinion similarities:
	%For binary random variables $f(v_1), f(v_2), \dots, f(v_n)$, 
    the {\em opinion similarity} $\sigma_{ij}$ for nodes $v_i$ and $v_j$ is defined as the probability that 
	$f(v_i)$ and $f(v_j)$ have the same values.
%Intuitively, the above defined similarity would help us to partition the nodes likely to hold the same opinions together.
%In fact, in the next section, we will show our key result that knowing pairwise similarities is
%enough for us to reduce the optimization problem to a graph partitioning problem
%	(Theorem~\ref{theorem:objective function}).

With the objective function and inputs settled, we are now ready to define our optimization problem:
    
\begin{definition}\label{def:OPS}
    (Optimal Partitioned Sampling) 
    Given a vertex set $V=\{v_1, v_2, \dots, v_n\}$, sample size budget $r<n$, and
    opinion similarity $\s_{ij}$ between every pair of nodes $v_i$ and $v_j$,
    the {\em Optimal Partitioned Sampling} (OPS) problem is to find the optimal partition $\mathcal{P}^*$ of $V$, 
    %with the corresponding sample size allocation, 
    such that the
    partitioned sampling method % as given in Method~\ref{al:partitioned}
    using $\mathcal{P}^*$ achieves the minimum 
    expected sample variance, i.e.,  $\mathcal{P}^* = \argmin_{\cal P} \E_M[\Var_S(\hat f_{\it part}({\cal P}))]$, where $\cal P$ takes among all partitions of
    $V$ with $r$ samples.
%    Suppose that a social network $G=(V,A)$ follows the \model{} opinion evolution model
%    with inward probabilities $p_1, p_2, \dots, p_n$ and Poisson rates $\lambda_1, \lambda_2, \dots, \lambda_n$.
%    Given the sample size budget $r$, the {\em Optimal Partitioned Sampling}
%    problem is to find the optimal partition $\mathcal{P}$ of $V$ with
%    the corresponding sample size allocation, such that when we use
%    partitioned sampling method as given in Algorithm~\ref{al:partitioned}
%    with the above partition $\mathcal{P}$ as input, the
%    expected sample variance $\E_M[\Var_S(\hat f_{\it part}({\cal P}))]$
%    is minimized.
\end{definition}

We remark that the OPS problem requires all pairwise opinion similarities as inputs so as to make the problem well-defined.
We will address the issue of handling missing or inaccurate opinion similarities 
	in Section \ref{section: discussion of similarity}, and show that partitioned sampling still has outstanding performance.
%
%	theoretical
%	aspects, opinion evolution model, and experimental evaluation in later sections.


%However, obtaining accurate similarities may not be easy in some cases.   %which may be hard to obtain in the real world.
%After solving the original OPS problem, we will propose several ways to handle the cases that opinion similarities are not accurate or even missing in Section \ref{section: discussion of similarity}.

==> content/sampling.tex <==
\section{Solving the OPS Problem}\label{section: solving the OPS problem}

There are two issues involved in the OPS problem: 
    one is how to partition the vertex set $V$ into $K$ groups; 
    the other is how to allocate the subsample size in each group.
For simplifying the OPS problem, 
    we first consider a special kind of partitions that pick only one sample node in each group.

\begin{definition}
    A {\em simple partition} is a partition in which the subsample size of each group is equal to one.
\end{definition}

Simple partitions are important not only for the simplicity but also for the superiority.
%We will show later in Theorem \ref{theorem: simple is better} that one of the optimal partitions must be a simple partition.
We will later show in Theorem \ref{theorem: simple is better} that, for any non-simple partition $\cal P$,
	one can easily construct a simple partition based on $\cal P$ which is at least as good as $\cal P$.
Thus, we focus on finding the optimal simple partition.% for the OPS problem.

Our approach is constructing a weighted assistant graph $G_a$ whose vertex set is $V$,
	where the weight of edge $(v_i,v_j)$ is $w_{ij}=1-\s_{ij}$,
    and then connecting the OPS problem with a graph partitioning problem for the graph $G_a$.
For a simple partition $\mathcal{P}=\{(V_1,1), (V_2,1), \dots, (V_r,1)\}$ of $V$, 
    we use $\Vol_{G_a}(V_k)$ to denote the volume of the group $V_k$ in the graph $G_a$, 
    defined as $\Vol_{G_a}(V_k)=\sum_{v_i,v_j\in V_k} w_{ij}$.
We define a cost function $g(\mathcal{P})$ to be the sum of all groups' volumes in $G_a$, 
    namely, $g(\mathcal{P})=\sum_{k=1}^r \Vol_{G_a}(V_k)$.
Our major technical contribution is to show that
    minimizing the expected sample variance of partitioned sampling using any simple partition $\mathcal{P}$ 
    is equivalent to 
    minimizing the cost function $g(\mathcal{P})$, %the volume summation of all the groups in $G_a$,
	as summarized by the following theorem:

\begin{restatable}{theorem}{objective}\label{theorem:objective function}
    Given a vertex set $V$ with pairwise opinion similarities $\{\s_{ij}\}$'s and sample size $r$, 
%    we construct an assistant graph $G_a$ whose vertex set is $V$
%    and edge $(v_i,v_j)$'s weight $w_{ij}$ is $1-\s_{ij}$.
	for any simple partition ${\cal P}=\{(V_1,1), (V_2,1),$ $ \dots, $ $(V_r,1)\}$ of $V$, 
    $$\E_M[\Var_S(\hat f_{\it part}({\cal P}))] =g({\mathcal{P}})/2|V|^2.$$ 
%    where $g({\mathcal{P}})$ is the volume summation of all the groups of $\mathcal{P}$ in $G_a$.
    Thus, the optimal simple partition of $V$ minimizes the cost function $g({\mathcal{P}})$.
\end{restatable}

The proof of the theorem requires involved computation and is included in the supplemental material.
The intuition of the theorem is that, small cost function indicates small volume of each group, 
    which implies that the nodes within each group have high opinion similarities.
Theorem \ref{theorem:objective function} makes precise our intuition that 
    grouping people with similar opinions 
    %and then sampling in each group separately 
    would make partitioned sampling more efficient.
 


Theorem~\ref{theorem:objective function} provides the connection between 
the OPS problem and the graph partitioning problem.
In particular, it suggests that we can reduce the OPS
    problem to the following {\em Min-$r$-Partition} problem: given an undirected graph with non-negative edge weights, partition the graph into $r$ groups such that the sum
    of all groups' volumes is minimized.
However, Min-$r$-Partition is NP-hard to approximate to within any finite factor \cite{kann1997hardness}, 
and to the best of our knowledge, there is no approximation or heuristic algorithms in the literature.
The good news is that Min-$r$-Partition and its dual problem (Max-$r$-Cut) are equivalent in the exact solution, 
    and there exist both approximation and heuristic algorithms for Max-$r$-Cut.
%Given an undirected graph with non-negative edge weights, partition the graph into $r$ groups
%    such that the total edge weight of the cut (set of edges crossing different
%    groups) is maximized.
%In particular, 
\citet{maxkcut} 
propose a semi-definite programming (SDP) algorithm which achieves
$1-1/r + 2\ln r/r^2$ approximation ratio and is the best to date.
%There are only two heuristic algorithms \cite{zhu2013max,ma2015multiple} for Max-$r$-Cut in the literature.
We adopt the SDP algorithm to solve the OPS problem.
The SDP partitioning algorithm including the SDP relaxation
program is given in the supplemental material.
The drawback of the SDP partitioning algorithm is its inefficiency.
Thus we further propose a greedy algorithm to deal with larger graphs, which takes the idea from a heuristic algorithm for Max-$r$-Cut \cite{zhu2013max}.
%    which can be applied to larger graphs.

Given a simple partition $\mathcal{P} = \{(V_1,1), \ldots, (V_r,1)\}$
    and an external node $v_i$ which does not belong to $V_k$ for any $k\in[r]$,
    we define $\delta g_\ell(v_i,\mathcal{P})$ to be $g(\mathcal{P'})-g(\mathcal{P})$,
    where $\mathcal{P'}$ %is the simple partition of $V\cup \{v_i\}$ and
    is $\{(V_1,1), \ldots, (V_\ell\cup\{v_i\},1), \ldots, (V_r,1)\}$.
Thus $\delta g_\ell(v_i,\mathcal{P})$ represents the increase of the cost function when the external node $v_i$ is added to the group $V_\ell$ of $\mathcal{P}$.
The greedy algorithm (Algorithm \ref{al:greedy}) first assigns each ungrouped node $x_i$ to the group 
    such that the objective function $g(\mathcal{P})$ is increased the least.
After the first round of greedy assignment, the assignment procedure is repeated to further
    decrease the cost function, until some stopping condition holds, such as 
    the decrease is smaller than a predetermined threshold.
%Notice that the cost function is positive, 
%    and there exists a certain gap\footnote{The gap is $\min_{i,U,W}|\sum_{j\in U} w_{ij}-\sum_{k\in W} w_{ik}|$ where $U$ and $W$ are two subsets of $V$ satisfying $U\cup W \subseteq V\setminus \{v_i\}$ and $U\cap W = \emptyset$.} that the decrease in each round must be greater than, 
%    therefore, the cost function should no longer decrease after finite rounds.

%Min-$r$-Partition problem can also be formed as a game:
%    Each node $v_i$ has $r$ strategies and each strategy corresponds to a group which it chooses to belong to.
%    The payoff of $v_i$ choosing group $V_j$ is $-\sum_{v_k\in V_j}w_{ik}$.
%    The summation of all nodes' payoffs is the negation of the cost function, and is what we want to maximize.
%From this point of view, the final output of the greedy algorithm is a Nash equilibrium of the game.
%\wei{If we do not have the result on the Price of Anarchy of the game, we do not need to
%	mention it as a game.}

\begin{algorithm}[t]
    \caption{Greedy Partitioning Algorithm}\label{al:greedy}
    \begin{algorithmic}[1]
        \Require Graph $G_a$ with $n$ nodes, number of groups $r$. 
        \State Randomly generate a node sequence of all the nodes: $x_1$, $x_2$, \dots, $x_n$.
        \State Let $V_1=\ldots =V_r = \emptyset$. 
        \Repeat
        \For {$i\gets 1$ \textbf{to} $n$}
        \If{$x_i \in V_j$ for some $j\in [r]$}{ $V_j=V_j\setminus \{x_i\}$.}
        \EndIf
        \State $k \leftarrow \arg\min_{\ell\in [r]} \delta g_\ell(x_i, \{(V_1,1),\ldots, (V_r, 1)\})$
        \State $V_k \leftarrow V_k \cup \{x_i\}$.
        %        \State Assign $v_{s_i}$ to the group $V_k$ such that   $$\delta g_r(v_{s_i}, V_k) \leq \delta g_r(v_{s_i}, V_l), \forall l\in[r].$$
        \EndFor
        %\State Let ${\cal P} = \{(V_1,1),\ldots, (V_r, 1)\}$.
        \Until{a predetermined stopping condition holds.}
        \State \textbf{Output:}  Partition $\mathcal{P} = \{(V_1,1),\ldots, (V_r, 1)\}$.
    \end{algorithmic}
\end{algorithm}

The running time of one-round greedy assignment is $O(n+m)$ where $m$ is the number of edges in $G_a$. 
In our experiment, we will show that greedy partitioning %with a reasonable stopping condition
performs as well as SDP partitioning but could run on much larger graphs.
Theoretically, the performance of partitioned sampling using the simple partition generated by the greedy partitioning algorithm
    is alway at least as good as naive sampling,
    even using the partition generated after the first round of greedy assignment, 
    as summarized below:
%The following lemma shows that
%    partitioned sampling using the simple partition generated by the greedy partitioning algorithm always performs at least as well as the naive sampling, even using the partition generated only after the first round of greedy assignment.

\begin{restatable}{lemma}{greedy}\label{lemma:greedy vs naive}
    Given a vertex set $V$ with % $n$ nodes and 
	    sample size $r$, 
    %for any opinion assignment $f:V\rightarrow \{0,1\}$,
    partitioned sampling using the simple partition $\mathcal{P}$
    generated by the greedy partitioning algorithm (even after the first round)
    is at least as good as naive sampling. Specifically,
    \[
    \E_M[\Var_S(\hat f_{\it part}({\cal P}))] \leq 
    \E_M[\Var_S(\hat f_{\it naive}(V,r))].
    \]
\end{restatable}

We call a partition $\mathcal{P}'$ a {\em refined} partition of $\mathcal{P}$, if each group
	of ${\cal P}'$ is a subset of some group of $\mathcal{P}$.
Suppose we are given a partition $\mathcal{P}$ such that there exists some group which is allocated more than one sample. 
Then we can further partition that group by the greedy partitioning algorithm
    and finally obtain a refined simple partition of $\mathcal{P}$.
According to Lemma \ref{lemma:greedy vs naive}, 
    the refined simple partition should be at least as good as the original partition $\mathcal{P}$,
    summarized as below:

\begin{restatable}{theorem}{simple}\label{theorem: simple is better}
    For any non-simple partition $\mathcal{P}$, there exists a refined simple partition $\mathcal{P}'$ of $\mathcal{P}$, 
    which can be constructed efficiently,
    such that partitioned sampling using the refined simple partition $\cal P'$ is 
    at least as good as partitioned sampling using the original partition $\cal P$. Specifically,
        \[
        \E_M[\Var_S(\hat f_{\it part}({\cal P}'))] \leq 
        \E_M[\Var_S(\hat f_{\it part}({\cal P}))].
        \]
\end{restatable}

Theorem \ref{theorem: simple is better} shows the superiority of simple partitions, and justifies that it is enough for us to only optimize for partitioned
	sampling with simple partitions.

\subsection{Dealing with Inaccurate Similarities}\label{section: discussion of similarity}
When accurate opinion similarities are not available, 
    one still can use a {\em balanced partition}
	(i.e., all groups have the exact same size) to achieve as least good sampling result as naive sampling, % for any similarity input,
    summarized as below:
	
\begin{restatable}{theorem}{balanced}\label{thm:balancedpartition}
	Given a vertex set $V$ with $n$ nodes and sample size $r$ where $n$ is a multiple of $r$, partitioned sampling using any balanced simple partition $\mathcal{P}$ %of $V$
		is at least as good as naive sampling. That is,
	    $\Var_S(\hat f_{\it part}({\cal P})) \leq 
	    \Var_S(\hat f_{\it naive}(V,r))$ holds for any fixed opinions $f(v_1)$, \dots, $f(v_n)$.
\end{restatable}

Theorem \ref{thm:balancedpartition} provides a safety net showing that partitioned sampling would not hurt sampling quality. 
Thus we can always use the greedy algorithm with a balance partition constraint to achieve better sampling result.
The result will be further improved if opinion similarities get more accurate.

Furthermore, in the experiment on the real-world dataset (Section \ref{section: experimental evaluation}), 
    we artificially remove all the opinion similarity information (set as 0.5) between disconnected individuals, and perturb the rest opinion similarities more than 30\%, to simulate the condition of missing and inaccurate similarities. 
The experimental result shows that the performance of the greedy algorithm with perturbed inputs is quite close to the performance of the greedy algorithm with exact inputs.
This demonstrates the robustness of our greedy algorithm in the face of missing and inaccurate opinion similarity data.

Moreover, since real-world social interaction can be characterized well by opinion evolution models, 
    we adapt a well-known opinion evolution model and give an exact computation of opinion similarity based on the model in the next section.
The model essentially provides a more compact representation than pairwise similarities.

